Which Modality should I use -- Text, Motif, or Image? : Understanding Graphs with Large Language Models

Our research integrates graph data with Large Language Models (LLMs), which, despite their advancements in various fields using large text corpora, face limitations in encoding entire graphs due to context size constraints. This paper introduces a new approach to encoding a graph with diverse modalities, such as text, image, and motif, coupled with prompts to approximate a graph's global connectivity, thereby enhancing LLMs' efficiency in processing complex graph structures. The study also presents GraphTMI, a novel benchmark for evaluating LLMs in graph structure analysis, focusing on homophily, motif presence, and graph difficulty. Key findings indicate that the image modality, especially with vision-language models like GPT-4V, is superior to text in balancing token limits and preserving essential information and outperforms prior graph neural net (GNN) encoders. Furthermore, the research assesses how various factors affect the performance of each encoding modality and outlines the existing challenges and potential future developments for LLMs in graph understanding and reasoning tasks. All data will be publicly available upon acceptance.

==> tex/tables.tex <==
%------------------------------------------

%\textcolor{red}{ishaan add the table and what the figure means  }table {edge representation setting, prompt }
%adj+x 
%Result means ??
\begin{table*}[ht]
\centering
\scriptsize
\begin{tabular}{p{0.1\textwidth}p{0.6\textwidth}p{0.3\textwidth}}
\toprule
Edge Representation & Prompt Associated & Explanation \\
\midrule
% Example row 1
Adjacency List & Task : Node Label Prediction (Predict the label of the node marked with a ?, given the adjacency list information as a dictionary of type "node:node neighborhood" and node-label mapping in the text enclosed in triple backticks. Response should be in the format ""Label of Node = <predicted label>"". 
If the predicted label cannot be determined, return ""Label of Node = -1"") \newline
```Adjacency list: {1558: [2339, 2340], 2339: [1558, 2340], 2340: [2339, 1558]}
Node to Label Mapping : Node 2339: Label 3| Node 2340: Label ?| Node 1558: Label 3| ```

&
None \\

% Example row 2
GML & Task : Node Label Prediction (Predict the label of the node marked with a ?, given the graph information in the form of a GraphML structure in the text enclosed in triple backticks. 
\{explanation\}
Response should be in the format ""Label of Node = <predicted label>"". If the predicted label cannot be determined, return ""Label of Node = -1"") \newline
```GraphML: graph [\newline
  \hspace*{0.2cm}node [\newline
    \hspace*{0.4cm}id 2339\newline
    \hspace*{0.4cm}label 3\newline
  \hspace*{0.2cm}]\newline
  \hspace*{0.2cm}node [\newline
   \hspace*{0.4cm} id 2340\newline
   \hspace*{0.4cm} label ?\newline
  \hspace*{0.2cm}]\newline
  \hspace*{0.2cm}node [\newline
   \hspace*{0.4cm} id 1558\newline
   \hspace*{0.4cm} label 3\newline
  \hspace*{0.2cm}]\newline
  \hspace*{0.2cm}edge [\newline
  \hspace*{0.4cm}  source 2339\newline
   \hspace*{0.4cm} target 1558\newline
  \hspace*{0.2cm}]\newline
  \hspace*{0.2cm}edge [\newline
   \hspace*{0.4cm} source 2339\newline
   \hspace*{0.4cm} target 2340\newline
  \hspace*{0.2cm}]\newline
]\newline
``` &
A GraphML format consists of unordered sequence of node and edge elements enclosed within []. Each node element has a distinct id and label attribute contained within []. 
Each edge element has source and target attributes contained within [] that identify the endpoints of an edge by having the same value as the node id attributes of those endpoints. The node label information is embedded within the structure meaning no node-label mapping is needed.\\

% Example row 3
GraphML & Task : Node Label Prediction (Predict the label of the node marked with a ?, given the graph information in the form of a GraphML structure in the text enclosed in triple backticks. \{explanation\}
Response should be in the format ""Label of Node = <predicted label>"". If the predicted label cannot be determined, return ""Label of Node = -1"") \newline
```GraphML: <graphml xmlns=http://graphml.graphdrawing.org/xmlns xmlns:xsi=http://www.w3.org/2001/XMLSchema-instance \newline xsi:schemaLocation=http://graphml.graphdrawing.org/xmlns \newline  http://graphml.graphdrawing.org/xmlns/1.0/graphml.xsd>
  <graph edgedefault=undirected>\newline
  \hspace*{0.2cm}  <node id=2339 label=3 /> \newline
  \hspace*{0.2cm}  <node id=2340 label=? />\newline
  \hspace*{0.2cm}  <node id=1558 label=3 />\newline
  \hspace*{0.2cm}  <edge source=2339 target=1558 />\newline
  \hspace*{0.2cm}  <edge source=2339 target=2340 />\newline
  </graph>\newline
</graphml>``` &
A GraphML file consists of an XML file containing a graph element, within which is an unordered sequence of node and edge elements. Each node element should have a 
distinct id attribute as well as its label, and each edge element has source and target attributes that identify the endpoints of an edge by having the same value as the id attributes of those endpoints. The node label information is embedded within the structure meaning no node-label mapping is needed. \\

Edgelist & Task : Node Label Prediction (Predict the label of the node marked with a ?, given the edge connectivity information and node-label mapping in the text enclosed in triple backticks. Response should be in the format ""Label of Node = <predicted label>"". If the predicted label cannot be determined, return ""Label of Node = -1"") 
```Edge connections (source node - target node): Node 85328 is connected to Node 158122. Node 158122 is connected to Node 167226. 
Node to Label Mapping : 
Node 85328: Label 16| Node 158122: Label ?| Node 167226: Label 16| ``` &
None \\

GraphML + Text & Task : Node Label Prediction (Predict the label of the node marked with a ?, given the graph information in the form of a GraphML structure in the text enclosed in triple backticks. 
\{explanation\}
Response should be in the format ""Label of Node = <predicted label>"". If the predicted label cannot be determined, return ""Label of Node = -1"") \newline
```GraphML: <graphml xmlns=http://graphml.graphdrawing.org/xmlns xmlns:xsi=http://www.w3.org/2001/XMLSchema-instance \newline xsi:schemaLocation=http://graphml.graphdrawing.org/xmlns \newline  http://graphml.graphdrawing.org/xmlns/1.0/graphml.xsd>
  <graph edgedefault=undirected>\newline
   \hspace*{0.2cm} <node id=2339 label=Neural\_Networks /> \newline
   \hspace*{0.2cm} <node id=2340 label=? />\newline
   \hspace*{0.2cm} <node id=1558 label=Neural\_Networks />\newline
   \hspace*{0.2cm} <edge source=2339 target=1558 />\newline
   \hspace*{0.2cm} <edge source=2339 target=2340 />\newline
   \hspace*{0.2cm} <edge source=2340 target=1558 />\newline
  </graph>\newline
</graphml>``` &
A GraphML file consists of an XML file containing a graph element, within which is an unordered sequence of node and edge elements. Each node element should have a 
distinct id attribute as well as its label, and each edge element has source and target attributes that identify the endpoints of an edge by having the same value as the id attributes of those endpoints. \\

Adjacency List + Text & Task : Node Label Prediction (Predict the label of the node marked with a ?, given the adjacency list information as a dictionary of type ""node:node neighborhood""
and node-label mapping in the text enclosed in triple backticks. Response should be in the format ""Label of Node = <predicted label>"". If the predicted label cannot be determined, return ""Label of Node = -1"") \newline
```Adjacency list: {1558: [2339, 2340], 2339: [1558, 2340], 2340: [2339, 1558]}
Node to Label Mapping : 
Node 2339: Label Neural\_Networks| Node 2340: Label ?| Node 1558: Label Neural\_Networks| ``` &
None \\

\bottomrule
\end{tabular}
\caption{Summary of edge representations with their associated prompts and explanations.}
\label{tab:edge_representations}
\end{table*}

%--------------------------------------------------------





